Overpredictive Signal Analytics in Federated Learning: Algorithms and Analysis

Edge signal processing facilitates distributed learning and inference in the client-server model proposed in federated learning. In traditional machine learning, clients (IoT devices) that acquire raw signal samples can aid a data center (server) learn a global signal model by pooling these distributed samples at a third-party location. Despite the promising capabilities of IoTs, these distributed deployments often face the challenge of sensitive private data and communication rate constraints. This necessitates a learning approach that communicates a processed approximation of the distributed samples instead of the raw signals. Such a decentralized learning approach using signal approximations will be termed distributed signal analytics in this work. Overpredictive signal approximations may be desired for distributed signal analytics, especially in network demand (capacity) planning applications motivated by federated learning. In this work, we propose algorithms that compute an overpredictive signal approximation at the client devices using an efficient convex optimization framework. Tradeoffs between communication cost, sampling rate, and the signal approximation error are quantified using mathematical analysis. We also show the performance of the proposed distributed algorithms on a publicly available residential energy consumption dataset.

==> Linked-files/02-Model.tex <==
\section{System Model and Background Concepts} \label{sec:prob_setup}
% Topic Sentences for the flow
%+ FL architecture
%+ on-device computation
%+ cloud aggregation
%+ signal class description - smooth differentiable signals
%+ optimization framework - convex cost function
%+ Think of adding boundedness on the signal -- if it helps in the analysis
%+ Need to avoid self-plagiarism
In this section we describe the signal model for overpredictive signal
analytics, and provide the background concepts useful for the related
mathematical analysis.  
%
\subsection{Distributed Signal Model}
%+ D client devices, and a central server (show figure)
%+ each client records a time series signal (continuous signal)
%+ we will assume p-times differentiability
%+ each device communicates an approx

Consider a distributed client-server model consisting of $D$ clients and a
central server, as described by the federated learning architecture shown in
Figure~\ref{fig:SCApp}. Each client device records a continuous-time signal
represented as $f_1(t), f_2(t), \ldots, f_D(t)$. Without loss of generality we
will assume that the recorded signals have a bounded support in the interval $[0,1]$.
For the ensuing analysis, we assume that these signals are $p$-times
differentiable, where $p \geq 1$. The signals at the client devices are to be
communicated to the central server to learn a global model.
However, due to the rate constrained client-server communication channel, the
devices only communicate an approximate signal, which will be denoted as
$\widehat{f}_1(t), \widehat{f}_2(t),\ldots,\widehat{f}_D(t)$.
% -- 
\begin{figure}[!hbt]
  \centering
  \includegraphics[scale=0.8]{SCApp-mod}
  \caption{\label{fig:SCApp} The federated learning system model for distributed
  signal analytics. In this model, $D$ client devices communicate an
  approximation of the recorded signals, and the central server pools these
  signals to obtain useful signal analytics such as the histogram,
  aggregate signal or a clustering of the devices.}
  %
\end{figure}
% 
\subsection{Fourier Basis Representation}
% + Fourier (our analysis is based on this) and Polynomial (Legendre is used in
%sim studies)
%+ Fact used -- Fourier coefficients decay
In this first exposition of the study of distributed signal
approximation in a federated learning model, will use the Fourier basis
representation for the signals at the client devices. That is, each recorded
signal at the clients can be represented by a Fourier series, 
%
\begin{align*}
  f_i(t) = \sum_{k = -\infty}^{\infty} a_i[k] \exp(j 2 \pi k t), \quad t \in
  [0,1], 
\end{align*}
%
where $i \in \{1,2, \ldots,D\}$. It will be assumed that $f_i(0) = f_i(1)$, which
is due to the periodicity requirement of the Fourier series representation.
Since the signals at the clients are assumed to $p$-times differentiable, we
observe a polynomial decay in the Fourier series coefficients of the signals,
which is stated in the fact below.
%
\begin{fact}[Sec~2.3,\cite{mallat2008}]%[Spectral property of smooth signals]
%
\label{lem:regularity} 
%
A signal $f(t), t \in [0,1]$, with $f(0) = f(1)$, is $p$-times differentiable
if its Fourier coefficient~$a[k]$ satisfies the condition,
%
 \begin{align}
%
|a[k]| \leq \frac{C}{|k|^{p+1+\varepsilon}} \quad \text{ for some }
C, p, \varepsilon >0. \nonumber
%
\end{align}
%
\end{fact}
%
\subsection{Mathematical Formulation and Related Definitions}
% + At devices - statement of the envelope constraint and the objective (L-2
% norm is assumed in this work)
% + At the server - Global Model of the approx functions - these global models
% can be histograms, peak energy demand - that is required for grid planning

For ths signal approximation, we consider the $L$ length bandlimited
approximation of the signals, $f_i(t)$ for $i \in \{1,2,\ldots,D\}$, given by
the Fourier series,
%
\begin{align} \label{eq:Fourierapp}
  \widehat{f}_i(t) = \sum_{k= -L}^{L} b_i[k] \exp(j 2 \pi kt) \quad \text{ for } t \in
  [0,1], 
\end{align}
%
where the coefficients $b_i[k]$ for $k \in \{-L,\ldots,L\}$, will be a function
of $a_i[k], k \in \zZ$. In particular, the approximation coefficients $b_i[k]$
are chosen such that it minimizes the approximation error measured with respect
to distance metric $d(.)$, such as ${\cal L}_1$, ${\cal L}_2$ or ${\cal
L}_\infty$ norm, subject to an overprediction constraint. Mathematically, this
is stated as,
%
\begin{align} \label{eq:opt_d_measure}
  \argmin_{\widehat{f}_i(t)} d(f_i(t),\widehat{f}_i(t)) \quad \text{ subject to }
  \widehat{f}_i(t)  \geq f_i(t).
\end{align}
%
Since the Fourier basis is orthogonal, the problem now translates into an
equivalent optimization in terms of the coefficients $a_i[k]$'s and $b_i[k]$'s.
For instance, when the distance metric is the ${\cal L}_2$
norm, the equivalent optimization is
%
\begin{align}
  \argmin_{b_i[k]} \sum_{k = -L}^{L} \left|a_i[k] -
  b_i[k]\right|^2 \;\; \text{ subject to }
  \widehat{f}_i(t)  \geq f_i(t).
\end{align}
%
The constraint in the considered optimization problem always ensures an
over-prediction of the true signal, hence the signal approximation obtained by
this method will be called the \textit{envelope approximation}. For simplicity,
we will denote the envelope approximation of a signal $f(t)$ by
$\widehat{f}_{\env}(t)$.
%
\subsection{Distance measures of interest}
%
For the overpredictive signal approximation, we will construct an envelope for
the signal recorded at each client device. The envelope approximation
$\widehat{f}_{\env}(t)$ of the signal $f(t)$ is obtained by solving the
optimization problem described in \eqref{eq:opt_d_measure}, with respect to a
distance metric $d(.)$ defined over the signal space. In this paper, the ${\cal
L}_1$ and ${\cal L}_2$ distance measures will be analyzed, and the ${\cal
L}_\infty$ formulation will be used to derive performance bounds.  Using the
Fourier representations of $\widehat{f}_{\env}(t)$ (akin
to~\eqref{eq:Fourierapp}, with the subscript indices dropped) and $f(t)$, and
the envelope property $\widehat{f}_{\env}(t) \geq f(t)$ it can be seen that,
%
\begin{align}
%
  \|\widehat{f}_{\env}-f\|_1 & = b[0] -a[0],\label{eq:L_1} \\[2ex]
%
  \|\widehat{f}_{\env}- f \|_2^2 = & \sum_{|k| \leq L} |b[k] -a[k]|^2 + \sum_{|k|>L}
	|a[k]|^2 \label{eq:L_2} \\[2ex]
%
  \|\widehat{f}_{\env}- f\|_\infty \leq & \sum_{|k| \leq L} |b[k] -a[k]| + \sum_{|k|>L}
|a[k]| \label{eq:L_inf} 
\end{align}    
% 
For ease of notation, the signal approximation error corresponding to
the ${\cal L}_1$, ${\cal L}_2$ and ${\cal L}_\infty$ distance measures will be
denoted by $\SA_1$, $\SA_2$ and $\SA_\infty$ respectively. The upperbound in
\eqref{eq:L_inf} will be used to show the performance bounds of envelope
approximations in Section~\ref{subsec:DC_boost}.

% --------- END OF SECTION ON SYSTEM MODEL --------- %


==> Linked-files/03-Algorithms.tex <==
\section{Algorithms for Overpredictive Analytics}
\label{sec:Algo}
%
In this section we revisit the distributed signal approximation application
using federated learning illustrated in Fig.~\ref{fig:SCApp}, where there are
$D$ devices and a central server. We discuss the algorithmic scheme for
performing signal analytics in a federated learning setting, where each device
reports an envelope approximation of the signal observed. The optimization
program implemented at the client devices and the signal analytics performed at
central server are discussed below. 

\subsection{At the Clients}
The optimization problem of interest at the client devices, is to
determine the best possible signal approximation, which forms an envelope of
the true signal. This can be stated as,
%
\begin{align}
%
  \min \SA_q := \int_{0}^1 \left| \widehat{f}(t) - f(t) \right|^q \mbox{d}t \mbox{
subject to } \widehat{f}(t) \geq f(t) \label{eq:sa1sa2}
%
\end{align}
%
for $q = 1, 2$, where the above minimizations are over $\widehat{f}_1(t),
\ldots, \widehat{f}_D(t)$. These device level analytics problems can be efficiently
solved, by using the equivalent forms of the function norms in the Fourier
domain, discribed in \eqref{eq:L_1} and \eqref{eq:L_2}.

For $q=1$, the above envelope approximation formulation will become a
\textit{linear program}, since the cost function in the Fourier representation
is the difference of the zero frequency components of the envelope and true signal.
%
When $q=2$ the problem is equivalent to a \textit{quadratic program with linear
constraints}, with the objective described by the squared error of the Fourier
coefficients within bandwidth $L$. Both $q=1$ and $q=2$, has linear inequality
constraints due to the envelope overprediction criteria. Since linear programs
are relatively easier to implement, the client devices with limited hardware
can choose to solve ${\cal L}_1$ optimization problem over the ${\cal L}_2$
problem.
%
\subsubsection*{Envelope Optimization with Discrete-time Signals}
In practice, the recorded client device signals are available at $n$ discrete time
samples. Since the true signal values are unknown at all times except the
sampled points, the set of inequality constraints in discrete-time case is a finite
subset of the envelope constraints in the continuous time case. Hence, the
discrete-time optimization yields a lower cost than the continuous-time
optimization. A related analysis of the discrete-time envelope optimization in
the context of TV whitespace application, along with Mean Squared Error (MSE)
performance is discussed in~\cite{Kumar:2017}. More detailed analysis of the
discrete time envelope optimization is presented in Sec~\ref{sec:Main_results}.
%
%
\subsection{At the server}
The signal approximations obtained from the clients will be combined at the
server to learn the signal analytics of interest.  In general a signal analytic
is a function over the envelope approximations $\widehat{f}_1(t),
\widehat{f}_2(t), \cdots, \widehat{f}_N(t)$. Examples of such analytics will
include the aggregate function, $\widehat{s}(t) := \sum_i \widehat{f}_i(t)$, or
a statistical quantity such as the empirical CDF, 
%
\begin{align}
  \widehat{F}_N(x) := \frac1N \sum_{n=1}^{N} \mathbbm{1}_{(-\infty,x]}(\widehat{f}(t_n)),
\end{align}
%
where $\mathbbm{1}{(-\infty,x]}(Y)$ represents the $0$--$1$ indicator function for the
probability event $\{Y \leq x\}$, and $t_n$ for $n \in \{1,2,\ldots,N\}$ represents
the time samples in the interval $[0,1]$.
%
It is known that several statistical properties can be inferred using this
classical Glivenko-Cantelli estimate of the CDF~\cite{Wainwright:2019}. 
%
Since the Glivenko-Cantelli estimate satisfies the uniform convergence
property, at the server there exists an implicit minimization of an empirical
loss function involving the true and estimated CDFs, i.e. the objective function,
%
\begin{align}
	\|\widehat{F}_N(x) - F(x)\|_{\infty},
\end{align}
%
is minimized by when $\widehat{F}_N(x)$ is the Glivenko-Cantelli estimate of
$F(x)$. This minimization task conforms with the definition of federated
optimization~\cite{McMahan:2017}.
%
Application of CDF estimation based signal analytics will be discussed
in the section~\ref{sec:exp}.
%
\subsection{Algorithm sketch for over-predictive signal analytics}
%
% + assume each device has capability to compute the envelope
It is assumed that each client device in the federated learning model works in a
distributed manner. To ensure $\widehat{f}_i(t) \geq f_i(t)$ for $i \in
\{1,2,\ldots, D\}$, we propose that each device can perform envelope
approximation of its observed signal.  The following steps are
proposed for obtaining a bandwidth-$L$ approximation $\widehat{f}_i(t)$ of $f_i(t)$:
%
\begin{enumerate}
%
\item Each device $i$ records its individual signal $f_i(t)$, computes its
	envelope $\widehat{f}_{i,\env}(t)$, using the envelope optimization
		\eqref{eq:sa1sa2}, and communicates the $(2L+1)$ Fourier
		coefficients to the server.
%
\item Using Fourier coefficients from each client device, the server calculates
	a global model (or statistic) of interest, denoted as
		$G_{\mbox{\footnotesize
    server}}\left(\widehat{f}_{1,\env}, \widehat{f}_{2,\env},\ldots,\widehat{f}_{D,\env}\right)$.
%
% \item Since $\widehat{s}_{\env}(t) \geq s(t)$; so, the proposed analytics
% $\SA$
% can be computed based on $\widehat{s}_{\env}(t)$.
%
\end{enumerate}
%

% It can be seen that the optimal distributed scheme for the independent devices
% is to transmit its own optimal individual envelope, that is
% $\widehat{f}_{i,\opt}(t) = \argmin_{f_{i,\env}(.)} \|\widehat{f}_{i,\env}
% -f_i\|$.
Signal envelope calculation in Step~1 above is outlined next. For ${\cal L}_1$
distance (see~\eqref{eq:L_1}), it will be calculated as,
%
\begin{align}
%
\mbox{minimize } & b[0] - a[0] \nonumber \\
%
  \mbox{subject to } & \vec{b}^{\;T} \Phi(t) \geq f(t), 
%
\end{align}
%
where $\Phi(t) = [\exp(-2\pi L t), \ldots, \exp(2 \pi Lt)]^T$ and $\vec{b} =
(b[-L], \ldots, b[L])^T$ are the Fourier series coefficients of the envelope
approximation. The above linear program with linear constraints is solvable
efficiently~\cite{Kumar:2017}. For ${\cal L}_2$, the cost
function $b[0] - a[0]$ is replaced by the quadratic cost in~\eqref{eq:L_2}.

As $L$ is increased, the envelopes $\widehat{f}_{i, \env}(t)$ become more
proximal to their target $f_i(t)$. It is expected that the approximation errors,
$\SA_1$ and $\SA_2$ will decrease as $L$ increases.  However, analyzing the
dependence of $\SA_q, q = 1, 2$ versus $L$ is difficult. Accordingly, a na\"{i}ve
envelope approximation will be used to analyze the fundamental bounds
on their tradeoff.


==> Linked-files/04-Main-results.tex <==
\section{Performance Bounds on Optimal Envelope Approximation\label{sec:Main_results}}
%
In this section, we analyze the performance of the $L$ bandwidth envelope
approximation. In particular, we provide an upper bound for the envelope
approximation error, using the idea of na\"{i}ve envelope approximation scheme,
described below .
%
\subsection{A Na\"{i}ve Envelope Approximation Scheme}
%
\label{subsec:DC_boost}
%
First consider a single client device, $i=1$ in isolation.  Let $f_{1,\proj}(t)$
be the orthogonal projection of $f_1(t)$ on the span of $\exp{(j2\pi kt)}$ for
$|k| \leq L$.  Then $f_{1,\proj}(t) = \sum_{|k|\leq L} a_1[k] \exp({j2\pi kt}).$
The na\"{i}ve envelope approximation scheme is as
follows~\cite{Maheshwari:2015}:
%
\begin{align} 
%
f_{1,\env}(t) = f_{1,\proj}(t) + C_0, \label{eq:naive_app}
%
\end{align}
%
where $C_0 = \|f_1 - f_{1, \proj}\|_\infty$. Using the triangle inequality, 
%
\begin{align}
%
C_0  \leq \sum_{|k|>L} |a_1[k]| \leq \sum_{|k|>L} \frac{C}{|k|^p}, \qquad p>1.
\label{eq:C0bound}
%
\end{align}
%
For $p > 1$~\cite[Sec.~2.2]{Bhatia:1993}, we can show that, $C_0 =
O\left(\frac{1}{L^{p-1}}\right)$.
%
% -----------------/ (Main Result) Envelope Approximation Analysis\-----------------
%
\subsection{Envelope Approximation Analysis}
% For what class is the naive scheme good.
In this section we answer the question -- \textit{for what class of signals is the
na\"{i}ve envelope approximation scheme good?} The result stated below shows
that there exist a certain class of signals for which the na\"{i}ve
approximation is order optimal to the optimal envelope scheme, while using
${\cal L}_1$ or ${\cal L}_2$ norm minimization.

In the result stated below we use the notation $\SA_q$ to denote the optimal
envelope approximation error (see \eqref{eq:L_1}), and the notation $\SA'_q$ to
be the approximation error corresponsing to the na\"{i}ve envelope approximation
in~\eqref{eq:naive_app}, where $q\in \{1,2\}$ according to the ${\cal L}_1$ or
${\cal L}_2$ cost metric.

%
\begin{theorem}
%
%[Naive approx. scheme achieves optimality for some signal classes}]
%
\label{th:main}
% write in a less intimidation manner
  %Let $\SA_q$ be the optimal envelope approximation error computed with ${\cal
  %L}_q$-norm based distance metric, and $\SA'_q$ be the approximation error
  %corresponding to the na\"{i}ve approximation in~\eqref{eq:naive_app}. 
	%The approximation error of the optimal envelope signal, $\SA_q$, is
	%order optimal to the approximation error of the na\"{i}ve envelope
	%signal, $\SA'q$ for some class of signals, where $q=1,2$. That is,
%
%	There exist a class of signals such that for $q = 1, 2$, the optimal envelope
%	approximation error $\SA_q$ has the same order of magnitude as that of
%	error corresponding to the na\"{i}ve approximation, $\SA'_q$. That is,
	The approximation errors of the optimal envelope signal and the
	na\"{i}ve envelope signal, \textit{viz.} $\SA_q$ and $\SA'_q$
	respectively for $q \in \{1,2\}$, are shown to be order optimal for a
	specific class of $p$-times differentiable signals as stated below.
	%
	\begin{enumerate}
		\item[(i)] The approximation error of the optimal ${\cal L}_2$
			envelope signal, $\SA_2$, is order optimal to the
			approximation error of the na\"{i}ve envelope signal,
			$\SA'_2$ for the class of $p$-times differentiable
			signals where Fourier coefficients,
			$|a_1[k]|=\frac{1}{|k|^p}$ for $|k|>L$.  That is,
			%
			\begin{align}
				%
			1 \leq \frac{\SA'_2}{\SA_2} \leq
				\left(1+\frac{1}{L}\right)^{2p-1}.  \nonumber
				%
			\end{align}
			%
		\item[(ii)] The approximation error of the optimal ${\cal L}_1$
			envelope signal, $\SA_1$ is the same as the
			approximation error of the na\"{i}ve envelope signal,
			$\SA'_1$ for the class of $p$-times differentiable
			signals with Fourier coefficients, $a_1[k] \geq 0$
			(non-negative) and $a_1[k]=a_1[-k]$ (symmetric) for all $k
			\in \zZ$. That is, 
			%
			\begin{align} 
				%
				\SA_1 = \SA'_1 = 2 \sum_{k>L} a_1[k]. \nonumber 
				%
			\end{align}
	\end{enumerate}
\end{theorem}
%
The detailed proof is shown in~\underline{\ref{app:order_optimal}}.

\noindent \textit{Remark}: The above result is shown for one (that is $D=1$)
client device. For $D$ clients with a sum signal analytic at the server (that
is $\widehat{s}(t) := \sum_{i=1}^D \widehat{f}_{i}(t)$), $\SA_1$ as well as
$\SA'_1$ scale linearly with $D$. In contrast, $\SA_2$ and $\SA'_2$ will scale
quadratically with $D$. Thus in both ${\cal L}_1$ and ${\cal L}_2$ norm based
error, the ratio between the approximation errors will remain the same, as in
the $D= 1$ case discussed in the proof.

\subsection{CDF of the Envelope Signal Approximation}
%
The CDF is a useful signal analytic to determine various statistical functions,
especially in a distributed learning setting such as federated learning.
Functions of the CDF estimates are beneficial in estimating customer usage
statistics such as mean, median or peak demand in the electricity smart
metering illustrated in Fig.~\ref{fig:Block_Dia}. By invoking
Therorem~\ref{th:main}, we derive performance bounds on the estimated CDF
obtained from the envelope approximation algorithms (see Sec.~\ref{sec:Algo}).
Let $F_X(x)$ denote the CDF of the actual signal $X(t)$ and let
$F_{X_{\env}}(x)$ be the CDF of the envelope signal approximation,
$\widehat{X}_{\env}(t)$, with $(2L+1)$ Fourier coefficients. In the result
below, we characterize an upper bound on the pointwise difference between the
actual and the estimated CDFs, as stated below.
%
\begin{theorem}
	The pointwise difference between the CDF of the actual signal, $F_X(x)$ and the
	CDF of the envelope signal approximation, $F_{\widehat{X}_{\env}}(x)$, with
	$(2L+1)$ Fourier coefficient is bounded by,
	%
	\begin{align}
		F_X(x) - F_{\widehat{X}_{\env}}(x) \leq \frac{C}{L^{\frac{2p-1}{3}}},
	\end{align}
	%
	where $C=\left(4^{\frac13} + 2\times 4^{-\frac23}\right)\frac{f_{X,\max}^{2/3}}{(2p-1)^{1/3}}$ and $f_{X,\max} := \begin{aligned}\max_x \left[\frac{d F_X(x)}{d x}\right]\end{aligned}$.
\end{theorem}
The proof of this result is available in \underline{\ref{app:Comm_Accuracy_Tradeoff}}
%

\subsection{Effect of Subsampling on CDF estimate}

In practice, signals are obtained as discrete samples over a finite interval.
Thus, it is essential to understand how envelope approximation can be performed
over signal samples and evaluate the tradeoff between the envelope
approximation error and the sampling rate. In this connection, we will consider
the aspect of signal sampling while limiting the discussion to the ${\cal L}_2$
distortion. However, a similar analysis also extends to the ${\cal L}_1$
distortion metric. The envelope signal approximation problem posed in
\eqref{eq:sa1sa2} is reformulated to reflect the finite signal sample
assumption as described below. If $\vec{b}_{\opt}$ represents the minimizer of
${\cal L}_2$ distance metric applied in \eqref{eq:sa1sa2}, then we define, 
%
\begin{align}
	\vec{b}_{\app,n} & :=\argmin_{\vec{b}}  \sum_{|k|\leq L} |b[k]-a[k]|^2 + \sum_{|k|>L} |a[k]|^2 \nonumber \\
	& \text{subject to} \quad \widehat{f}_{\env}(t_n) \geq f(t_n), \quad \forall \; t_n \in \left\{0,\frac1n, \frac2n,\ldots, 1\right\}, \label{eq:discrete_L_2}
\end{align}
%
where $n$ is a positive integer denoting the number of signal samples. Also, we
define the approximately optimal envelope signal, $f_{\app,n}(t):=
\vec{b}_{\app,n} \Phi(t)$. The above formulation in \eqref{eq:discrete_L_2} has
only finite inequality constraints as against the infinite inequality
constraints in \eqref{eq:sa1sa2}. Due to the relaxation of the envelope
constraints attributed to signal sampling, the ${\cal L}_2$ cost of the approximately
optimum envelope is lesser than the optimum envelope. This difference in the
${\cal L}_2$ cost of the envelope error, for the infinite envelope constraint
and the sampled envelope constraint relaxation as characterized
in~\cite{Kumar:2017} is written as,
%
\begin{align}
	\sum_{|k| \leq L} \left[\left|b_{\opt}[k] - a[k]\right|^2 - \left|b_{\app,n}[k] - a[k]\right|^2\right] \leq 2 (b_{\app,n}[0] - a[0]) \left(\frac{c+c'}{n}\right) + o(1/n). \label{eq:discrete_bound}
\end{align}
The constants $c$ and $c'$ in the above upperbound expression corresponds
to the maximum slopes of the actual signal and the approximately optimal
envelope signal respectively. That is, $|f'(t)|\leq c$ and
$|f'_{\app,n}(t)|:=c'$. The upperbound on $c'$ is shown to be $2\pi L
\|f\|_{\infty}$, in \cite{Kumar:2017}. 
% + first formulate the problem; stick onto L_2 cost; cost function can be
% mapped;
% + introduce the variant - the appopt and subopt methods; (follows similar proof steps)
% + estimate the difference between subopt and optimal envelope;
% + cite the ArXiv paper by AK
%\textbf{Result from Arxiv paper-AK} The difference between the suboptimal
%envelope and the optimal envelope is $O(1/n)$, where $n$ is the number of
%samples used~\cite{Kumar:2017}.

Let $F_X(x)$ be the CDF of the actual signal, $X(t):= \sum_{k \in \zZ}
A[k]\exp(j2 \pi k t)$ for $t \in [0,1]$.  Further, let $F_{X_{\app,n}}(x)$ be
CDF of the envelope signal approximation with the subsampled constraints,
$\widehat{X}_{\app,n}(t): = \sum_{|k| \leq L} B_{\app,n}[k] \exp(j 2 \pi k
t)$ for $t \in [0,1]$, where the set of coefficients $\{B_{\app,n,i}[k]: -L
\leq k \leq L\}$ is as defined in~\eqref{eq:discrete_L_2}. An upperbound
between the pointwise difference of the two CDFs is shown below, 
%
\begin{theorem}
	The pointwise difference between the CDF of the actual signal, $F_X(x)$
	and the CDF of the subsampled envelope signal approximation, $F_{X_{\app,n}}(x)$,
	with $(2L+1)$ Fourier coefficient is bounded by,
	\begin{align}
		F_X(x) - F_{X_{\app,n}}(x) \leq C \times \left\{\frac{4}{2p-1} \frac{1}{L^{2p-1}} + 8\mu_{\app,n}\frac{c+c'}{n} + o(1/n)\right\}^{1/3},
	\end{align}
	where $C = \left(2^{\frac13} + 2^{-\frac23}\right) f_{X,\max}^{2/3}$
	and $f_{X,\max} := \begin{aligned}\max_x \left[\frac{d F_X(x)}{d
	x}\right]\end{aligned}$. The constant, $\mu_{\app,n} =
	\eE\left[B_{\app,n}[0]-A[0]\right]$, where $B_{\app,n}[0]$ and $A[0]$
	are the zero frequency components corresponding to the signals
	$\widehat{X}_{\app,n}(t)$ and $X(t)$ respectively.
%
\end{theorem}
The proof of this result is available in~\underline{\ref{app:Subsampling_CDF}}.


==> Linked-files/05-Experiments.tex <==
% This is the experiments section linked to the paper
% This section needs to be rewritten to avoid self plagiarism
\section{Experimental Results and Discussion}\label{sec:exp}
%
\subsection{Electricity Consumption Dataset}
%+ Basic Setup
%+ Tradeoff - Comm vs Approx Error
%+ CDF Estimation
%+ Effect on subsampling (s = 2, 3 etc) - peak violation error
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.45]{fig_L1}
  \includegraphics[scale=0.45]{fig_L2}
  \caption{\label{fig:L2_Signal} The sum of signals obtained by distributed
	envelope approximation schemes are compared with the ground truth
	signal, when the number of coefficients communicated are $L =72$. Plot
	(a) and (b) consider ${\cal L}_1$ and ${\cal L}_2$ cost functions
	respectively. It is observed that the optimal envelope approximation
	signal estimates the peak energy demand regions.}
	%
\end{figure}
%
%
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.55]{figL2_Tradeoff}
  \caption{\label{fig:L2_Tradeoff} This plot depicts the tradeoff between
	normalized root mean-squared (RMS) error and the number of Fourier coefficients
  transmitted per device. The distributed envelope approximation scheme based
	on ${\cal L}_1$ and ${\cal L}_2$-norms converge to the zero error as
	the number of communicated coefficients increase. The plot also shows the RMS error for the  na\"{i}ve envelope signal and the MSE optimal signal (which is devoid of any envelope constraints).}
\end{figure}
%
% Simplified plots that convey meaning
%+ Dataset 1 : (Fourier Basis)
%+ residential energy consumption - 39 homes, 24 average consumption data to be
%reported
%+ Use of Fourier basis -- 2 envelope method .. naive and (opt) envelope
%approximation (come up with a good notation), also MSE can be communicated
%+ tradeoff between mean squared error and number of coefficients is analyzed
%(both L1 and L2)
%+ CDF plot(s), quantile table, variation with number of devices (stick to L1)
To analyze the effect of envelope approximation in a federated learning model,
we have conducted experiments on an available electrical energy consumption
dataset~\cite{Mammen:2018}, consisting of hourly electricity consumption of 39
users from a residential building. The experimental results discussed here, are
conducted on those users having atleast 30 days of data with synchronized
timestamps -- which turned out to be 37 users. In the original dataset,
energy (in W-hr units) measurements corresponding to three phases were
available. However, for the doing the experimental study we have considered only a
single phase (represented as W3 in the dataset). %Due to space constraints, we
%have restricted the experimental results and discussions to the ${\cal L}_2$
%norm based envelope approximation.

\vspace{1ex}
\textbf{Hardware/Software Specifications}: The simulations on the dataset were
performed in a PC with the Processor model -- Intel(R) Core(TM) i3-2310M
CPU @ 2.10GHz, 2100 Mhz, 2 Core(s), RAM 6 GB; and implemented in MATLAB 2015b
(Windows platform) using the standard curve fitting toolbox and CVX package (ver
2.1).

\subsection{Communication Cost and Approximation Error Tradeoff}
% to rewrite
The tradeoff between the number of communicated Fourier coefficients and the
envelope approximation error, is studied by considering a sum signal analytic
(or the sum of user energy consumptions) to be learned at the central server.
Each Fourier coefficient communicated to the server is a real valued floating
point number which is typically 4 Bytes (or 32 bits).  In this setting, each
client device (i.e. the 37 users) sends the Fourier coefficients of the
envelope approximation, representing 30 days of hourly energy consumption, or
720 signal samples~(refer Fig.~\ref{fig:L2_Signal} for the time-series plot of
the sum signal analytic). In the tradeoff plot shown in
Fig.~\ref{fig:L2_Tradeoff}, we notice that there is a graceful degradation of
the relative root mean-squared (RMS) error of the optimal envelope
approximation scheme for both ${\cal L}_1$ and ${\cal L}_2$ cost functions, as
the number of Fourier coefficients transmitted are reduced. It is observed that
the distributed signal approximation schemes approache an error of zero when
720 Fourier coefficients are transmitted.  However, the naive approximation,
which adds only a constant to the projection based Fourier representation,
fails to capture the envelope trend for the considered dataset.  For reference,
we have marked two extremum points -- first corresponding to the least
communication scheme(that is $L=1$), and the second where all coefficients are
communicated (that is $L=360$). The ${\cal L}_1$ cost function results in a
relatively lower RMS error compare to ${\cal L}_2$, which is due to the better
time-series fit of ${\cal L}_1$ as shown in Fig.~\ref{fig:L2_Signal}. Further,
we observe that the relative approximation error of classical MSE minimizer
(that is, without the envelope constraint) is lower than distributed envelope
by one order of magnitude.
%
\subsection{Cumulative Distribution Function based Signal Analytics}
%
In this experimental study, we allow the central server to learn the CDF of the
signal samples from the approximate signals reported by the individual clients.
From the learned CDF, the central server can infer statistical
properties, which are symmetric functions of the data, to measure the electricity
usage patterns at the client devices. %\hl{For instance, the mean (mode or
%median) consumption, or the peak demand can be inferred}. 
In Fig.~\ref{fig:L2_CDFs}, we illustrate the convergence of the CDF estimate
obtained from the envelope approximation samples to the baseline CDF, obtained
by a model which access to all the raw signal samples from all clients. At low
approximation levels, for instance $L =36$, the estimated CDF of the envelope
scheme is much away from the true CDF. As we increase the number of communicated
Fourier coefficients, the gap between the CDFs is observed to reduce. Another
important observation is that the overprediction based CDFs (envelope as well as
the naive approximation schemes) always appears to the right of the true CDF.
This is because of the envelope constraint at the devices.
%
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.45]{figCDFs_L2}
  \caption{\label{fig:L2_CDFs} Plot illustrating the convergence of the
  empirical CDFs of the envelope signal to the actual CDF (obtained by pooling
	the raw signal samples at server) for the ${\cal L}_2$ cost function.
	The optimum as well as the na\"{i}ve envelope signal CDFs always
	appears towards the right of the true CDF, due to the envelope
	constraint. }
  %
\end{figure}

Using these CDF plots, the quantile estimates can also be inferred. In
Table~\ref{tab:quantile}, we compare the quantiles of the true CDF with the
quantiles of the CDF estimates. %at different approximation levels.
It is noted that the higher order quantiles deviate much as compared to the
lower ones, which is attributed to the overprediction constraint at the devices.
The accuracy of the quantile estimates in Table~\ref{tab:quantile} can be
improved by an appropriate choice of the basis representation. This shall be
addressed in a future work.
%
\begin{table}[!hbt]\scriptsize
  \centering
  \caption{\label{tab:quantile} A comparison of the quantiles of the true signal
  with the envelope approximation signal}
  \renewcommand{\arraystretch}{1.5}
  \begin{tabular}{@{}cccccclccc@{}}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\bf Quantile}} &
	  \multicolumn{1}{c}{\multirow{2}{*}{\parbox{1cm}{\centering \bf  Actual Signal}}} &
	  \multicolumn{1}{c}{\multirow{2}{*}{\parbox{1.5cm}{\centering \bf Cost Function}}} &
	  \multicolumn{3}{c}{\centering \bf Envelope Signal} & &  \multicolumn{3}{c}{\centering \bf Na\"{i}ve Envelope Signal} \\
	  \cline{4-6} \cline{8-10}
    %
	  \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & $L = 36$ & $L = 180$ & $L =324$ & & $L = 36$ & $L = 180$ & $L = 324$\\
    \midrule 
	  \multirow{2}*{$\mathbf{10\%}$} & \multirow{2}*{$0$} & ${\cal L}_1$ & $0.21$ & $10^{-6}$ & $10^{-7}$ & & \multirow{2}{*}{$66.34$} & \multirow{2}{*}{$39.19$} & \multirow{2}{*}{$7.79$}\\ \cline{3-6} & & ${\cal L}_2$ & $3.39$ &  $0.80$ & $0.11$ & & & &  \\
	  \midrule
    %
	  \multirow{2}*{$\mathbf{50\%}$} & \multirow{2}*{6.09} &  ${\cal L}_1$ & $19.25$ & $10.12$ & $6.78$ & & \multirow{2}{*}{$754.85$} & \multirow{2}{*}{$410.91$} & \multirow{2}{*}{$116.05$} \\ \cline{3-6} & &  ${\cal L}_2$ & $65.36$ & $27.55$ & $13.36$  & & & & \\
	  \midrule
    %
	  \multirow{2}*{$\mathbf{90\%}$} & \multirow{2}*{204.53} & ${\cal L}_1$ & $429.59$ & $272.41$ & $225.71$ & & \multirow{2}{*}{$2162.7$} & \multirow{2}{*}{$1229.2$} & \multirow{2}{*}{$514.11$}\\ \cline{3-6}  & & ${\cal L}_2$ & $431.21$ & $268.6$ & $218.42$ & & & & \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Effect of Subsampling}
%
In practice, as the signal acquisition in the edge device will not be a
recording a continuous signal, we will investigate the effect of signal
sampling on the envelope approximation algorithms. Since the dataset considered
here is already discrete time-series with $720$ samples, we will see the effect
of subsampling on the various performance metrics. In particular, for this
experimental study we consider three performance error metric, \textit{viz.}
(i) Wasserstein distance between the estimated envelope CDF and the actual CDF,
(ii) Number of envelope constraint violations with respect to the actual $720$
samples, and (iii) Peak envelope error after subsampling. We have used the 1-D
Wasserstein distance between the CDF of the envelope signal and the CDF of the
actual signal, that is defined as,
%
\begin{align*}
	{\cal W}(X,\widehat{X}_{\env}) := \int_0^1\left|F_{X}^{-1}(z) - F_{\widehat{X}_{\env}}^{-1}(z)\right| dz,
\end{align*}
%
where $F_{\widehat{X}_{\env}}(x)$ is the envelope signal CDF and $F_{X}(x)$ is
the true signal CDF. The number of envelope constraint violations and the peak
envelope error are computed based on the pointwise difference between the sum
of envelope approximated time-series and the sum of actual time-series. In
Fig~.\ref{fig:Subsamp-figs}, we show the various performance metrics
considering the ${\cal L}_1$ cost function for different subsampling rate,i.e. $S
\in \{1,2,4,8\}$. At a subsampling rate of $S$, the number of envelope
constraints is $720/S$. From Fig.~\ref{fig:Subsamp-figs}~(a), it is observed
that subsampling by considering alternate signal samples, i.e. $S=2$, reduces
the Wasserstein distance between the CDFs of the envelope signal and the true
signal, when compared with the envelope without subsampling, i.e. $S=1$. This
is attributed to the envelope constraint relaxation upon subsampling, which
results in a lesser minima for the same objective function. Since the CDF of
the MSE approximation signal does account for the envelope constraints the
Wasserstein distance approach zero with increasing approximation coefficients,
as shown in Fig.~\ref{fig:Subsamp-figs} (a). 

However, subsampling introduces violations of the envelope constraint as shown
in Fig.~\ref{fig:Subsamp-figs}~(b)-(c). Both the percentage of envelope
constraint violations and the peak error due to envelope constraint violation
increase with the number of approximation coefficients $L$. This is because of
the effect of signal aliasing and signal overfitting introduced due to
subsampling. Further it is noted that the signal reconstruction from subsampled
time-series fails when the number of Fourier coefficients is more than the
total number of signal samples, i.e. $2L+1 \geq 720/S$. In this case envelope
approximation algorithm fails to solve the optimization program owing to rank
deficiency. This effect is shown in  Fig.~\ref{fig:Subsamp-figs} (a), where the
Wasserstein distance returned by the solver starts to increase at $L=45$ for
$S=8$ and $L=90$ for $S=4$. For $S=2$, the rank violation will begin at $L=180$
although not shown in the plot.

The rank deficiency also results in an abrupt increase in envelope errors as
depicted in Fig.~\ref{fig:Subsamp-figs} (b)-(c). The tradeoff
between the sampling rate, Wasserstein's distance and the envelope violations,
suggests that envelope approximation algorithm should be limited to $2L+1 <
720/S$, where the aliasing effects due to subsampling are small. A similar
trend is seen to hold when the ${\cal L}_1$ cost function is replaced by the
${\cal L}_2$ cost function. We make a comparison between the envelope
approximation algorithms of ${\cal L}_1$ and ${\cal L}_2$ cost functions based
on the three performance metrics for $S=2$ in Table~\ref{tab:envViola}. Due to
the relatively poor signal fitting of the ${\cal L}_2$ compared to ${\cal L}_1$
as shown in Fig.~\ref{fig:L2_Signal}, the Wasserstein distance is more for
${\cal L}_2$ cost. However the number of envelope errors and the peak envelope
error is reduced because of the higher envelope constraint guard region at
lower signal amplitudes for the ${\cal L}_2$ approximation. Thus, for the low
envelope approximation regime, i.e.  $L=10$ to $L=50$, it is suggestive to
employ the ${\cal L}_2$ approximation algorithm when subsampling, as the
envelope constraint violations are better controlled. 

%However we observe that the peak envelope violation is of
%the same order, across different envelope approximations. This is shown in
%Figure~\ref{fig:Subsamp-figs} (b).
%
\begin{figure}[!hbt]
  \centering
  \includegraphics[scale=0.5]{fig1_wasserstein}
  \includegraphics[scale=0.5]{figL1_viola}	
  \includegraphics[scale=0.5]{figL1_peak}	
	\caption{\label{fig:Subsamp-figs} The figures depict the effect of subsampling on the ${\cal L}_1$ cost based envelope approximation based on three performance metrics: (a) Wasserstein distance of estimated envelope CDF and true CDF, (b) percentage of envelope violations at different subsampling rates, (c) peak envelope error due to subsampling.}
  %
\end{figure}
%
%\begin{table}[!hbt]\scriptsize
%  \centering
%  \caption{\label{tab:envViola} Envelope contraint violations upon subsampling }
%  \renewcommand{\arraystretch}{1.4}
%	\begin{tabular}{@{}cccc@{}}
%    \toprule
%		\multicolumn{1}{c}{\multirow{4}{*}{\parbox{2.72cm}{\centering\bf Number of \newline Approximation \newline Fourier Coefficients \newline $L$}}} &
%    \multicolumn{3}{c}{\bf Number of Envelope Violations}  \\
%	  \cline{2-4} 
%    %
%		%\multicolumn{1}{p{2.5cm}}{} 
%		&  \multicolumn{1}{p{1cm}}{\centering {Envelope \newline Signal \newline $S=2$}} &  \multicolumn{1}{p{1cm}}{\centering {Envelope \newline Signal \newline $S=1$}}& \multicolumn{1}{p{1cm}}{\centering{MSE\newline Signal \newline $S=1$}} \\
%%   \multicolumn{1}{c}{$L$} 		&  \multicolumn{1}{c}{$S=2$} &  \multicolumn{1}{c}{$S=1$} & \multicolumn{1}{c}{$S=1$} \\
%    \midrule
%	  $9$ & $8 \;(1.11\%)$ & $0$ & $308 \;(42.78\%)$ \\
%    %
%	  $18$ & $12 \;(1.67\%)$ & $0$ & $348 \;(48.33\%)$ \\
%    %
%	  $36$ & $19 \;(2.64\%)$ & $0$ & $339 \;(48.08\%)$\\
%    %
%	  $72$ & $30 \;(4.17\%)$ & $0$ & $336 \;(46.67\%)$ \\
%    %
%	  $108$ & $46 \;(6.39\%)$ & $0$ & $345 \;(47.91\%)$ \\
%    %
%	  $144$ & $47 \;(6.53\%)$ & $0$ & $349 \;(48.47\%)$ \\
%    \bottomrule
%  \end{tabular}
%\end{table}
%
\begin{table}[!hbt]\scriptsize
  \centering
	\caption{\label{tab:envViola} Comparison of different error metric for the ${\cal L}_1$ and the ${\cal L}_2$ cost functions, assuming $S=2$ subsampling}
  \renewcommand{\arraystretch}{1.5}
	\begin{tabular}{@{}cccccccccc@{}}
    \toprule
	%
	\multicolumn{1}{c}{\multirow{2}{*}{\parbox{2cm}{\centering\bf
		Error Metric}}} & \multicolumn{1}{c}{\multirow{2}{*}{\parbox{1.5cm}{\centering\bf
		Cost Function}}} & \multicolumn{8}{c}{ \centering \bf Envelope
		Approximation}  \\ 
	\cline{3-10} 
		\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & $L=10$ & $L=20$ & $L=30$ & $L=40$ & $L=50$ & $L= 60$ & $L=70$ & $L=80$ \\ 
	%
	\midrule 
		\multicolumn{1}{c}{\multirow{2}{*}{\parbox{2.5cm}{\centering\bf Wasserstein Distance}}} & ${\cal L}_1$ & $9725.63$ & $6396.24$ & $4775.37$ & $3390.32$ & $2906.97$ & $2370.42$ & $1913.22$ & $1670.10$ \\
		& ${\cal L}_2$ & $11378.52$ & $8051.19$ & $6050.24$ & $4403.93$ & $3867.93$ & $3220.06$ & $2725.07$ & $2400.25$ \\	
	%
	\midrule
	%
		\multicolumn{1}{c}{\multirow{2}{*}{\parbox{2.5cm}{\centering\bf Number of Envelope Violations}}} &  ${\cal L}_1$ &  $0$ & $1$ & $0$ & $4$ & $4$ & $6$ & $8$ & $10$ \\
		&  ${\cal L}_2$ & $0$ & $0$ & $0$ & $2$ & $2$ & $5$ & $6$ & $7$ \\	
		%
	\midrule
		\multicolumn{1}{c}{\multirow{2}{*}{\parbox{2.5cm}{\centering\bf Peak Envelope Error (in W-Hr)}}} &  ${\cal L}_1$ & $0$ & $408.26$ & $0$ & $1158.47$ & $1484.85$ & $1756.70$ & $2313.55$ & $2581.35$ \\
%		$0$ & $408.26$ & $0$ & $607.61$ & $925.62$ & $894.49$ & $1199.69$ & $1182.58$ \\
		& ${\cal L}_2$ & $0$ & $0$ & $0$ & $683.21$ & $793.70$ & $1271.43$ & $2044.13$ & $2363.26$ \\
		%$0$ & $0$ & $0$ & $356.36$ & $521.55$ & $799.26$ & $1116.81$ & $1135.05$ \\
		%
	\bottomrule
	\end{tabular}

\end{table}

    %

%\subsection{SVM based Envelope}
%+ Tradeoff between envelope constraint and MSE
%+ Effect of the Epsilon parameter (and noise)
%+ Subsampling effects
%+ Other basis representations - (wavelets) dictionary learning?
%+ Comparing with non-linear functions (linear-exponentials) 
%The SVM based envelope approximation has the tunable parameter $C_2$, which is
%the scaling factor of the envelope cost. For these experiments we have added
%zero-mean Gaussian noise of variance 100, and the value of $\varepsilon$ was
%fixed to be $5$. On varying $C_2$ we capture various performance metrics
%related to the envelope approximation. As $C_2$ increases, the number (or
%percentage) of envelope violation drops exponentially. In
%Figure~\ref{fig:SVM-figs}~(a), we show this trend for various values of $L$.
%The mean-square error for the envelope optimization increases initially and
%then saturates at a certain level. This can be attributed to the compliance
%with the envelope constraint after a certain threshold $C_2$. The mean-squared
%error decreases with finer envelope Fourier approximations, as depicted in
%Figure~\ref{fig:SVM-figs}~(b). In Figure~\ref{fig:SVM-figs}~(c), we show the
%number of data points within the $\varepsilon$-band. The figure suggest that
%the number of support vectors decreases with finer approximations. 
%%
%\begin{figure}[!hbt]
%  %
%  \centering
%  \includegraphics[scale=0.45]{SVM-fig-1}
%  \includegraphics[scale=0.45]{SVM-fig-2}
%  \includegraphics[scale=0.45]{SVM-fig-3}
%  \includegraphics[scale=0.45]{SVM-fig-4}
%	\caption{\label{fig:SVM-figs} \hl{(a) The number of envelope violations
%	as a function of the envelope penalty parameter $C_2$. (b) The effect
%	of $C_2$ on the mean-squared error. (c) Plot depicts the number of points within the $\varepsilon$-band for different levels of approximations. (d) Distance between CDFs}}
%  %
%\end{figure}


%\subsection{Other Extensions/Future Directions}
%+ Renewable Sources - Wind or Solar (underprediction)
%+ Hydrology dataset 
%+ Path planning for UAV
%+ Radar + Distance Estimation - quantizer?
%+ LSTM prediction to compare the computations

